DFM: Dialogue Foundation Model for Universal Large-Scale Dialogue-Oriented Task Learning

Building a universal conversational agent has been a long-standing goal of the dialogue research community. Most previous works only focus on a small set of dialogue tasks. In this work, we aim to build a unified dialogue foundation model (DFM) which can be used to solve massive diverse dialogue tasks. To achieve this goal, a large-scale well-annotated dialogue dataset with rich task diversity (DialogZoo) is collected. We introduce a framework to unify all dialogue tasks and propose novel auxiliary self-supervised tasks to achieve stable training of DFM on the highly diverse large scale DialogZoo corpus. Experiments show that, compared with models of the same size, DFM can achieve state-of-the-art or competitive performance on very rich cross-domain downstream dialogue tasks. This demonstrates that DFM largely extends the ability of unified dialogue pre-trained model.

==> limit.tex <==
\section*{Limitations}
A limitation regarding any work that conducts experiments with large pre-trained language models is the energy consumption and environmental impact, the current work included. However, the goal of this work is to improve the ability of dialogue understanding, knowledge distillation and dialogue generation. We hope that the benefits in future energy saved will outweigh the up-front costs of constructing the dialogue foundation models.

Another limitation is lack of the scale diversity of pre-trained dialogue foundation model in current version. We only train two different DFMs based on BART-base and T5-base. We leave this exploration for future work. We will try the proposed multitask learning method on larger pre-trained language models, like T5-large and T5-3B.

\section*{Ethical Considerations}
The collection of dialogue-oriented corpora is a big part of this work. As our dialogue foundation models are built upon the existing datasets, we follow the original copyright statements of collected 73 datasets and will further release our reformulated text-to-text data to the research community. All claims in this
paper are based on the experimental results. No demographic or identity characteristics information is used in this paper.
